Correlation-aware Unsupervised Change-point Detection via Graph Neural Networks

Change-point detection (CPD) aims to detect abrupt changes over time series data. Intuitively, effective CPD over multivariate time series should require explicit modeling of the dependencies across input variables. However, existing CPD methods either ignore the dependency structures entirely or rely on the (unrealistic) assumption that the correlation structures are static over time. In this paper, we propose a Correlation-aware Dynamics Model for CPD, which explicitly models the correlation structure and dynamics of variables by incorporating graph neural networks into an encoder-decoder framework. Extensive experiments on synthetic and real-world datasets demonstrate the advantageous performance of the proposed model on CPD tasks over strong baselines, as well as its ability to classify the change-points as correlation changes or independent changes. Keywords: Multivariate Time Series, Change-point Detection, Graph Neural Networks

==> background.tex <==
\section{Problem Definition}
\label{sec:background}
We are given a collection of multivariate time series data as $\{ \mathbf{X}_i \}$ with each $\mathbf{X}_i \in \mathbf{R}^{T\times N\times M}$, where $T$ is the time steps, $N$ is the number of variables and $M$ is the features of each variable.

% Mathematically, the set of time series data we observe is $\{ \mathbf{X}_i \}$, with each $\mathbf{X}_i$ a series of observations $\{\mathbf{x}^1, \mathbf{x}^2, \ldots, \mathbf{x}^T\}$ of $T$ time steps. The time series involves $N$ variables with $M$ features for each, such that $\mathbf{x}^t \in \mathbb{R}^{N \times M}$. We use $\mathbf{x}^t_i\in \mathbb{R}^M$ to denote the feature vector of variable $i$ at time $t$. Features are helpful to determine the dynamics of variables; however in real-world senario, not all dataset has additional features (such that $M=1$). In this case, we use `subsequence' as the feature vector, $\mathbf{x}^t_i = [x^t_i, x^{t+1}_i, \ldots, x^{t+K-1}_i]$ for some $K > 1$. $\mathbf{X}_i \in \mathbb{R}^{T \times N \times K}$ is also known as Hannkel matrix \cite{liu2013change}, which plays an important role in multivariate CPD \cite{kawahara2007change, moskvina2001application}.

We solve the CPD problem in retrospective setting by unsupervised learning. In retrospective setting, a complete time series $\mathbf{X}_i$ is given and a change-point at time step $t$ satisfies:
\begin{align*}
    \{ \mathbf{x}^1, \mathbf{x}^2, \ldots, \mathbf{x}^{t-1} \} &\sim \mathbb{P}(\mathbf{x}) \\
    \{ \mathbf{x}^{t}, \mathbf{x}^{t+1}, \ldots, \mathbf{x}^{T} \} &\sim \mathbb{Q}(\mathbf{x}) 
\end{align*}
Where $\mathbb{P}$ and $\mathbb{Q}$ denotes two different distributions. %Besides detecting when change-point happened, we are also interested in finding whether the difference between $\mathbb{P}$ and $\mathbb{Q}$ is because of independent change or correlation change.

In the following parts, We will introduce our methodology and architecture in Section \ref{sec:method} and show our experimental results and analysis in Section \ref{sec:synthetic} \ref{sec:real}.

% \section{Method}
% \label{sec:method}
% Our goal is to detect a change-point in multivariate time series as well as to categorize the detected property change into two types: independent change and correlation change. Our proposed Correlation-aware Dynamics Models (\ourmodelshort) disentangles the two types of changes based on two concepts in multivariate time series:

% \textbf{Dynamics} An inherent property of the system, e.g. physical laws, market supply \& demand, which controls the motion of independent variables.

% \textbf{Correlation} The interdependence between the variables, e.g. particle attraction, company cooperation, which is related to variable interactions.

% The value of a variable at each time step is determined by the law of dynamics and its correlation with other variables. Dynamics and correlations are ubiquitous in many systems, such as Brownian motion \& particle attraction or revenue growth \& company cooperation. The observed multivariate time series is result of both factors.
% %Different systems of time series may have different dynamics and correlation, which means that both of them should be learnt from downstream tasks instead of being defined by human assumptions. 
% Our \ourmodel model separates the effect of the two factors and from observed data by deep graph neural networks. Specifically, the encoder extracts the correlation from variables, and the decoder captures the dynamics rule from the values of time series. A change occurred in dynamics corresponds to an independent change, and a change in correlation corresponds to a correlation change. As a change-point could be a mixture of factors, the final prediction is an ensemble of both. 

   
% \subsection{Correlation Change}
% \label{subsec-correlation}
% In order to detect changes of correlation, the encoder of \ourmodel extracts an affinity matrix of variables at each time step, $\{\bm{A}^1, \bm{A}^2, \ldots, \bm{A}^T\}$ where $\bm{A}^t \in \mathbb{R}^{N \times N}$. Each cell in $\bm{A}^t$ is between $0$ and $1$, indicating how much they are related. The score of correlation change $s_r$ is calculated by the $L_1$ distance between two neighbor predicted relations:
% \[ s_{r}^t = \| \bm{A}^t - \bm{A}^{t-1}\| \text{, } t \ge 1 \] 

% \subsection{Independent Change}
%  The \ourmodel decoder estimates the expected value of time series in the future $k$ steps under the learnt dynamics rule. In a short period of time, if a system follows the dynamics rule, the expected value will be close to the observed value; If a system has experienced an abrupt independent change, those values will be different and the difference serves as a change-point score. Previous work \cite{chang2019kernel, ramakrishnan2019anomaly} uses forecasting method to calculate a change-point score, but only with a single point of horizon $h$. However, choosing a hyperparameter $h$ can be tricky. On the one hand, when $h$ is small, as illustrated in \cite{kipf2018neural}, a model can learn to copy the last observed value as the forecast value to achieve relatively low loss, which leads to performance degradation. On the other hand, when $h$ is large, the forecasting value will have large volatility \cite{lai2018modeling} causing a large variance in the change-point scores. To alleviate the extreme of both sides, we forecast a window in the future with size $k$. The independent change-point score $s_{d}$ is calculated by the distance of the expected value $\mathbf{\hat w}^t=\{\mathbf{\hat x}^{t+1}, \mathbf{\hat x}^{t+2}, \ldots, \mathbf{\hat x}^{t+k}\}$ and the observed value $\mathbf{w}^t=\{\mathbf{x}^{t+1}, \mathbf{x}^{t+2}, \ldots, \mathbf{x}^{t+k}\}$:
% \[ s_{d(t)} = \operatorname{Dist}( \mathbf{\hat w}^{t-1}, \mathbf{w}^{t-1}) \text{, } t \ge 1 \]
% where we use $\operatorname{MSE}$ as our choice for $\operatorname{Dist}$ function.

% \subsection{Ensemble of Changes}
% The encoder and decoder separately predict the scores for correlation changes and independent changes. A change-point occurred in a multivariate time series could result from one of them, or a mixture of both. In this study, we provide a simple way to ensemble the scores that yields good performance in practice. The ensemble score $\mathbf{s}_{en}$ is calculated by:
%     \[ \mathbf{s}_{en} = \operatorname{Norm}(\mathbf{s}_{r}) + \operatorname{Norm}(\mathbf{s}_{d}) \]
%     \[ \operatorname{Norm}(\mathbf{s}) = \frac{\mathbf{s} - u_s}{\sigma_s} \]
% where $u_x$ and $\sigma_x$ are mean and standard deviation of $x$.





==> framework.tex <==
\section{Model Architecture}
\label{sec:model}

\begin{figure*}[t!]
     \centering
     \includegraphics[width=\linewidth]{Img/encoder.png}
     \caption{\ourmodel Encoder: the encoder extracts correlation changes from multivariate time series, and outputs an affinity matrix at each step. The temporal encoding network captures time dependent features, and the spatial encoding network models relational features between variables.}
     \label{fig:enc}
\end{figure*}

In this section, we describe our \ourmodel architecture which has an encoder for correlation extraction and decoder for dynamics model.

We denote the time series from time $t_1$ to $t_2$ inclusively as $\bm{X}^{[t_1, t_2]}$. The encoder outputs a relation matrix $\bm{A}^t$ for each time step $t$. In our retrospective setting, we provide the entire time-series as input.

\begin{equation}
    \text{enc}_\phi(\bm{A}|\bm{X}) = \prod_{t=1}^T{\text{enc}_\phi({\bm{A}^t}|\bm{X}^{[1,T]})}
\end{equation}

The decoder reconstructs the time series by recovering the value $\bm{x}^{t+1}$ auto-regressively with $\bm{A}^t$ and $\bm{X}^{[1,t]}$. 

\begin{equation}
    \text{dec}_\theta(\bm{X}^{[2,T]}|\bm{A}) = \prod_{t=1}^T{\text{dec}_\theta(\bm{x}^{t+1}|\bm{X}^{[1,t]}, \bm{A}^t)}
\end{equation} 

The objective function of our autoencoder is:
\begin{equation}
    \mathcal{L} = \mathbb{E}_{\text{en}c_\phi({\bm{A|X}})}[\log \text{dec}_\theta(\bm{X}|\bm{A})]
\end{equation}

\subsection{Correlation Encoder}
We implement a graph neural network to capture pairwise interactions between variables in multivariate time series. Different from \cite{yang2018glomo, kipf2018neural, battaglia2016interaction}, which treat the underlying correlation map as static, we capture the a changeable relation at each time step.

As shown in Figure \ref{fig:enc}, the encoder calculates a correlation matrix $\bm{A}^t$ at each time step $t$, given the entire time-series $\bm{X}\in\mathbb{R}^{T\times N \times M}$, where $T$ is the number of time-steps, $N$ is the number of variables and $M$ is the number of features. We propose a temporal encoding layer (TE) to capture both temporal dependencies between $T$ steps and a spatial encoding layer (SE) to model the interaction between $N$ variables. Specifically, we alternative apply the TE and SE modules to progress incorporate the temporal feature and the correlation feature into the latent embeddings of each variable. Mathematically, for any two variables $i$ and $j$,

\begin{equation}
    \label{eq-encoder}
    \bm{Y} = \operatorname{TE_2}(\operatorname{SE}(\operatorname{TE_1}(\bm{X})))
\end{equation}

Finally, we predict the relation between every pair of variables by a 1-layer fully-connected network using the concatenation of the embeddings between them.
\begin{equation}
    \label{eq-fc-out}
    \bm{A}^t_{i,j} = \operatorname{Softmax}(\operatorname{FC}([\bm{Y}[t, i, :]; \bm{Y}[t, j, :]])) 
\end{equation}

The equation \ref{eq-encoder} and \ref{eq-fc-out} shows the structure of our encoder. 

In implementation, $\bm{Y}\in\mathbb{R}^{T\times N \times H}$ has the same first two dimensions $T$ and $N$ as $\bm{X}$, because both the spatial and temporal encoding layer will preserve the number of time-steps and variables. If we want to capture multiple relations in a time series, each $\bm{A}_{i,j}^t$ could be high dimensional vector representing the probability distribution on different types of edge. We apply Gumbel-Softmax \cite{jang2016categorical} to enforce sparse connections in the graphs and to reduce noise.

In the next sub-sections, we describe in details of our design of the TE and SE layers.

\subsubsection{Temporal Encoding Layer}
It is hard to detect the influence of the relation between variables by only observing a single time-step. Inferring the relation from a series of observations would be easier, because the difference between observations from different time-steps is usually informative. The TE layer captures both the long- and short-term dependencies. Take $\bm{X}\in \mathbb{R}^{T\times N \times M}$ as input, the TE layer will encode each of the $N$ variables separately and identically. In other words, we feed $N$ representations $\bm{X}[:, i, :]\in\mathbb{R}^{T \times M}$ into the TE layer in parallel, where $i={1,2,...,N}$. We propose two types of temporal encoding layer: the RNN\textsubscript{TE} and the Trans\textsubscript{TE}.

\paragraph{RNN\textsubscript{TE}} The recurrent neural networks are good at capturing temporal dependencies. Therefore, we use a bidirectional GRU network\cite{cho2014learning} as the RNN-based temporal encoder. We noticed that the bidirectional GRU, which captures both forward and backward time time steps, is empirically superior than unidirectional GRU. It indicates retrospective change-point detection gives more reliable predictions than the online change-point detection in our task. The following equations shows the encoded representation of the $i^{\text{th}}$ variable at the $t^{\text{th}}$ step is computed by concatenating the output from the two directions of GRU.  

\begin{equation}
    \overrightarrow{\bm{h}_i}^t = \overrightarrow{\text{GRU}}(\overrightarrow{\bm{h}_i}^{t-1}, \bm{X}[t, i, :])
\end{equation}
\begin{equation}
    \overleftarrow{\bm{h}_i}^t = \overleftarrow{\text{GRU}}(\overrightarrow{\bm{h}_i}^{t+1}, \bm{X}[t, i, :])
\end{equation}
\begin{equation}
    \bm{h}_i^t = [\overrightarrow{\bm{h}_i}^t, \overleftarrow{\bm{h}_i}^t]
\end{equation}

\paragraph{Trans\textsubscript{TE}} Although GRU is designed to combat the gradient vanishing problem, it still requires a long propagation path to capture long-range dependencies. A good alternative to solve the problem is by the Transformer model \cite{vaswani2017attention}, which uses a self-attention mechanism to aggregate information between any two embeddings. In this way, Transformer can be useful to capture both long- and short-term dependents. Both of the dependencies are crucial to our task, because local dynamics are reflected by short period of time, and correlations are revealed in a long time duration.

Similar to \cite{vaswani2017attention}, we use a positional encoding to incorporate the position information for TE. Then the embeddings are processed by a block consists of a multi-head self-attention layer and a feed-forward network, and each of them is followed by residual connection and layer normalization.

\subsubsection{Spatial Encoding Layer}
The TE layers itself may not be able to model the correlation between variables through time. To inject an inductive bias for relation learning, we use graph neural networks (GNN) \cite{kipf2016semi} to learn the correlation. The purpose of SE is to integrate the information among all variables at each time-step. As shown in Figure \ref{fig:enc}, the SE layer is orthogonal to the TE layer. We propose the following two types of modules: GNN\textsubscript{SE} and Trans\textsubscript{SE}. 

\paragraph{GNN\textsubscript{SE}} Similar to \cite{kipf2018neural}, we use the a message passing mechanism of GNN to aggregate information from neighbor nodes. The following equations show how the messages are passed in one layer of our GNN\textsubscript{SE}:
\begin{equation}
    \label{eq:agg}
 \bm{\tilde{h}}_{i,j} = f_e([\bm{x}_i;  \bm{x}_j])   
\end{equation}
\begin{equation}
\label{eq:com}
\bm{h}_{j} = f_v(\bm{x}_{j} + \sum_{i\neq j} \bm{\tilde{h}}_{i,j})
\end{equation}
Both $f_e(.)$ and $f_v(.)$ are MLPs. The $[;]$ represents the concatenation of vectors.

Graph-based models gather neighborhood information by an aggregation and combination process \cite{xu2018powerful}. Equation \ref{eq:agg} aggregates the neighborhood information and equation \ref{eq:com} combines the neighboring features by a summation. Graph networks are especially good at learning relations by sharing information from local to global. The learning complexity will be significantly decreased, compared to a fully-connected MLP \cite{xu2019what}. 

\paragraph{Trans\textsubscript{SE}} Transformer can also be considered as a graph-based model which operates on a fully-connected graph \cite{kool2018attention}, since the pairwise multi-head attention aggregates information from neighboring nodes. Compared to GNN, Transformer has additional well-designed structure of residual connection and layer normalization, which could be an advantage of Trans\textsubscript{SE} for spatial encoding. Similar to GCN\textsubscript{SE}, Transformer enables message exchanging among the multiple variables. However, the positional encoding layer is removed, because variables are order invariant.

\begin{figure}[ht!]
     \centering
     \includegraphics[width=\linewidth]{Img/decoder2.png}
     \caption{\ourmodel decoder: Given the correlation graph, the decoder recovers the expected value of time series from learnt dynamics.}
     \label{fig:dec}
\end{figure}

\subsection{Dynamics Decoder}
The decoder module learns the dynamics rule of a system, and recovers the expected value of time series. As shown in Figure \ref{fig:dec}, the decoder calculates the expected dynamics change at each time step, by $\text{dec}_\theta(\bm{x}^{t+1}|\bm{X}^{[1,t]}, \bm{A}^t)$. Since the dynamics are guided by the correlation, we also use a graph-based model to incorporate relational information into embeddings. For each relation type $k$, we have a distinct function $g^k_e(.)$ for the message passing. The functions $g^k_e(.)$ and $g_v(.)$ MLPs.

\begin{equation}
\bm{c}^t_{i,j} = \sum_k{\bm{A}^t_{i,j}}g_e^k([\bm{x}_i^t, \bm{x}_j^t])
\end{equation}
\begin{equation}
\bm{c}^t_{j} = g_v(\bm{x}_j + \sum_{i\neq j} \bm{c}^t_{i,j})
\end{equation}

$\bm{A}^t_{i,j,k} \in [0,1]$ represents the probability of the $k^{\text{th}}$ relation type. If the relation type vector $\bm{A}^t_{i,j}$ is one-hot, only one type of relation will be active. If $\bm{A}^t_{i,j}$ is a soft-max probability vector, it would calculate a distributed sum of the messages propagated through different types of relations.

Reconstructing time series performed by calculating the dynamic change with the help of MLP or RNN ($g_{\text{out}}$). MLP work be a simle choice if the feature vector of a variable is good enough to predict the dynamics; otherwise RNN is preferable to aggregate history information from time series. Together we have: 
\begin{equation}
    \bm{\mu}^{t+1}_j = \bm{x}^t_j+\Delta \bm{x}^{t}_{j} = \bm{x}^t_j + g_{\text{out}}(\bm{c}^{t}_{j})
\end{equation}
\begin{equation}
    \text{dec}_\theta(\bm{x}^{t+1}|\bm{X}^{[1,t]}, \bm{A}^t) = \mathcal{N}(\bm{\mu}^{t+1}, \sigma^2\bm{I})
\end{equation}

Then we can minimize the reconstruction error:
\begin{equation}
    \mathcal{L}_{rec} = \sum_j \sum_{t=2}^T \frac{\|\bm{x}^t_j-\bm{\mu}^t_j\|^2}{2\sigma^2}
\end{equation}

\subsection{Relation Smoothness Regularization}
Since change-points are sparse in time series, we don't expect sharp changes to occur too frequently between the encoded relations. We add an additional regularization loss to control the smoothness of relation and to prevent instability:

\begin{equation}
    \mathcal{L}_{smooth} = \frac{1}{T-1} \sum_{t=2}^T \|\bm{A}^t - \bm{A}^{t-1}\|_2^2 
\end{equation}
The final loss function is:
\begin{equation}
\mathcal{L} = \mathcal{L}_{rec} + \lambda \mathcal{L}_{smooth}
\end{equation}
where $\lambda$ controls the relative strength of smoothness regularization.
